Stochastic Model of Qudit Measurement for Superconducting Quantum Information Processing

The field of superconducting quantum computing, based on Josephson junctions, has recently seen remarkable strides in scaling the number of logical qubits. In particular, the fidelities of one- and two-qubit gates are close to the breakeven point with the novel error mitigation and correction methods. Parallel to these advances is the effort to expand the Hilbert space within a single device by employing high-dimensional qubits, otherwise known as qudits. Research has demonstrated the possibility of driving higher-order transitions in a transmon or designing innovative multimode superconducting circuits, termed multimons. These advances can significantly expand the computational basis while simplifying the interconnects in a large-scale quantum processor. This thesis provides a detailed introduction to the superconducting qudit and demonstrates a comprehensive analysis of decoherence in an artificial atom with more than two levels using Lindblad master equations and stochastic master equations (SMEs). After extending the theory of the design, control, and readout of a conventional superconducting qubit to that of a qudit, the thesis focuses on modeling the dispersive measurement of a transmon qutrit in an open quantum system using quadrature detections. Under the Markov assumption, master equations with different levels of abstraction are proposed and solved; in addition, both the ensemble-averaged and the quantum-jump approach of decoherence analysis are presented and compared analytically and numerically. The thesis ends with a series of experimental results on a transmon-type qutrit, verifying the validity of the stochastic model.

==> Makefile <==

#
# uclathes Makefile
# Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
#

FILES=README \
	demo.tex demo.dvi demo.pdf \
	demo_techreport.tex demo_techreport.pdf \
	thesis_spec.tex thesis_spec.pdf \
	uclathes.cls uclath12.clo uclathti.clo uclathma.clo \
	uclathes.bst Makefile

all:  latex ps pdf

tar: $(FILES)
	tar cvf uclathes.tar $(FILES)

tar.gz:
	@echo "Make all before doing make tar.gz"
	tar czvf uclathes.tar.gz $(FILES)

DVIPS=dvips
PS2PDF=ps2pdf14

latex latex.demo::
	latex demo

ps demo.ps::
	$(DVIPS) demo

pdf demo.pdf::
	$(PS2PDF) demo.ps demo.pdf

latex latex.demo_techreport::
	latex demo_techreport

ps demo_techreport.ps::
	$(DVIPS) demo_techreport

pdf demo_techreport.pdf::
	$(PS2PDF) demo_techreport.ps demo_techreport.pdf

latex latex.thesis_spec::
	latex thesis_spec

ps thesis_spec.ps::
	$(DVIPS) thesis_spec

pdf thesis_spec.pdf::
	$(PS2PDF) thesis_spec.ps thesis_spec.pdf

clean:
	rm *.aux *.toc *.lot *.lof *.dvi *.log *.ps

